H$^3$GNNs: Harmonizing Heterophily and Homophily in GNNs via Joint Structural Node Encoding and Self-Supervised Learning

Graph Neural Networks (GNNs) struggle to balance heterophily and homophily in representation learning, a challenge further amplified in self-supervised settings. We propose H$^3$GNNs, an end-to-end self-supervised learning framework that harmonizes both structural properties through two key innovations: (i) Joint Structural Node Encoding. We embed nodes into a unified space combining linear and non-linear feature projections with K-hop structural representations via a Weighted Graph Convolution Network(WGCN). A cross-attention mechanism enhances awareness and adaptability to heterophily and homophily. (ii) Self-Supervised Learning Using Teacher-Student Predictive Architectures with Node-Difficulty Driven Dynamic Masking Strategies. We use a teacher-student model, the student sees the masked input graph and predicts node features inferred by the teacher that sees the full input graph in the joint encoding space. To enhance learning difficulty, we introduce two novel node-predictive-difficulty-based masking strategies. Experiments on seven benchmarks (four heterophily datasets and three homophily datasets) confirm the effectiveness and efficiency of H$^3$GNNs across diverse graph types. Our H$^3$GNNs achieves overall state-of-the-art performance on the four heterophily datasets, while retaining on-par performance to previous state-of-the-art methods on the three homophily datasets.

==> sections/related.tex <==
\section{Related Work}
\label{sec:related}
\subsection{Learning on Heterophilic Graphs}

Heterophilic graphs are prevalent in various domains, such as online transaction networks ~\cite{pandit2007netprobe}, dating networks ~\cite{altenburger2018monophily}, and molecular networks ~\cite{zhu2020beyond}. Recently, significant efforts have been made to design novel GNNs that effectively capture information in heterophilic settings, where connected nodes possess dissimilar features and belong to different classes.

Some studies propose capturing information from long-range neighbors from various distance ~\cite{li2022finding, liu2021non, abu2019mixhop, pei2020geom, suresh2021breaking}. For example, MixHop ~\cite{abu2019mixhop} concatenates information from multi-hop neighbors at each GNN layer. Geom-GCN ~\cite{pei2020geom} identifies potential neighbors in a continuous latent space. WRGAT ~\cite{suresh2021breaking} captures information from distant nodes by defining the type and weight of edges across the entire graph to reconstruct a computation graph. 

Other approaches focus on modifying traditional GNN architectures to achieve adaptive message passing from the neighborhood ~\cite{chen2020simple, chien2020adaptive, yan2021two, zhu2020beyond}. For instance, GPR-GNN ~\cite{chien2020adaptive} incorporates learnable weights into the representations of each layer using the Generalized PageRank (GPR) technique, while H2GCN ~\cite{zhu2020beyond} removes self-loop connections and employs a non-mixing operation in the GNN layer to emphasize the features of the ego node.

Additionally, some papers approach the problem from spectral graph theory ~\cite{luan2021heterophily, bo2021beyond}, claiming that high-pass filters can be beneficial in heterophilic graphs by sharpening the node features between neighbors and preserving high-frequency graph signals.

However, these methods still heavily rely on labeled data, which is impractical for real-world datasets due to the significant manual effort required and the necessity of ensuring label quality. Furthermore, they are limited in their ability to effectively learn from the data itself without extensive supervision.



\subsection{Graph Representation Learning via SSL}
Self-supervised learning (SSL) has gained a lot of attention in the realm of graph graph representation learning. Graph SSL approaches are generally divided into two primary categories: graph contrastive learning and graph generative learning.

\subsubsection{Graph contrastive learning}
Contrast-based methods generate representations from multiple views of a graph and aim to maximize their agreement, demonstrating effective practices in recent research. For example, DGI~\cite{velivckovic2018deep} and InfoGraph~\cite{sun2020infograph} utilize node-graph mutual information maximization to capture both local and global information. MVGRL~\cite{hassani2020contrastive} leverages graph diffusion to create an additional view of the graph and contrasts node-graph representations across these distinct views. GCC~\cite{qiu2020gcc} employs subgraph-based instance discrimination and adopts the InfoNCE loss as its pre-training objective. GRACE~\cite{zhu2020deep} and GraphCL~\cite{you2020graph} learn node or graph representations by maximizing the agreement between different augmentations while treating other nodes or graphs as negative instances. BGRL~\cite{thakoor2021bootstrapped} contrasts two augmented versions using inter-view representations without relying on negative samples. Additionally, CCA-SSG~\cite{zhang2021canonical} adopts a feature-level objective for graph SSL, aiming to reduce the correlation between different views. These contrast-based approaches effectively harness the structural and feature information inherent in graph data, contributing to the advancement of self-supervised learning on graphs.

However, most of these methods are based on the homophily assumption. Recent works have demonstrated that SSL can also benefit heterophilic graphs. For instance, HGRL~\cite{chen2022towards} enhances node representations on heterophilic graphs by reconstructing similarity matrices to generate two types of feature augmentations based on topology and features. GraphACL~\cite{xiao2024simple}  predicts the original neighborhood signal of each node using a predictor. MUSE~~\cite{yuan2023muse} constructs contrastive views by perturbing both the features and the graph topology, and it learns a graph-structure-based combiner. GREET ~\cite{liu2022beyond} employs an edge discriminator to separate the graph into homophilic and heterophilic components, then applies low-pass and high-pass filters accordingly. However, these methods rely on the meticulous design of negative samples to provide effective contrastive signals. Moreover, although some approaches such as GREET and MUSE achieve impressive results, they require alternative training. This significantly increases computational overhead and may lead to suboptimal performance.

\subsubsection{graph generative learning}
Generation-based methods reconstruct graph data by focusing on either the features and the structure of the graph or both. Classic generation-based approaches include GAE ~\cite{kipf2016variational}, VGAE ~\cite{kipf2016variational}, and MGAE ~\cite{wang2017mgae}, which primarily aim to reconstruct the structural information of the graph, as well as S2GAE ~\cite{tan2023s2gae}. In contrast, GraphMAE ~\cite{hou2022graphmae} and GraphMAE2 ~\cite{hou2023graphmae2} utilize masked feature reconstruction as their primary objective, incorporating auxiliary designs to achieve performance that is comparable to or better than contrastive methods.

In the context of generative learning on heterophilic graphs, DSSL~\cite{xiao2022decoupled} operates under the assumption of a graph generation process, decoupling diverse patterns to effectively capture high-order information. Similarly, NWR-GAE ~\cite{tang2022graph} jointly predicts the node degree and the distribution of neighbor features. However, despite these innovative approaches, their performance on node classification benchmarks is often unsatisfactory~\cite{hou2022graphmae}.


